Dynamic Duos for Reliable Test-Time Adaptation: Two Models are Better than One

Test-time adaptation (TTA) updates a model on unlabeled test data to improve accuracy under distribution shift. However, a major obstacle to deploying TTA is that it can also reduce accuracy, and most TTA methods give no signal of failure. We show how to adapt Asymmetric Duos, which pair a larger model with a smaller model, for more reliable adaptation with minimal overhead. We find that a Duo is already more robust than its members even without adaptation. Adapting both members of the Duo can raise accuracy further, but one model can collapse while the other stays accurate, and the Duo's fixed combination keeps trusting both. We propose Dynamic Duos, which replace the Duo's fixed combination with a gate that re-weights the members on every batch using a label-free reliability estimate. We extend gating to resetting by using the same estimate to restore a collapsed member to its source weights while its partner keeps adapting. Dynamic Duos are compatible with any TTA update rule. On ImageNet-C with Tent, Dynamic Duos help most where adaptation fails: they gain $5.5$ points over a fixed combination for a Duo whose small member collapses. Where adaptation succeeds, Independent Dynamic Duos stay within $0.2$ points of the fixed combination on every corruption. On continual ImageNet-C, Dynamic Duos that Reset outperform or match scheduled resets and other baselines on all settings we evaluate.

==> tables/1_temperatures/tab_temperatures__frozen_bn__vitb16_convnextt.tex <==
\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{4.5pt}
    \caption{
    Temperatures and top-1 accuracy (\%) of the frozen Duo at severity 5 on episodic ImageNet-C. 
    Large / Small: \textbf{ViT-B/16 / ConvNeXt-T}. 
    $T_L^*, T_S^*$: the temperatures minimizing the NLL of the Duo on each stream, which define the corr.-wise oracle, and $T_L^*/T_S^*$ their ratio. 
    Clean TS $T_L = 1.11$, $T_S = 0.60$; Held-out TS $T_L = 0.72$, $T_S = 0.94$ .
     In the Average row, temperatures are geometric means.}
    \label{tab:temperatures:frozen_bn__vitb16_convnextt}
    \label{tab:oracles:frozen_bn__vitb16_convnextt}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l ccc cc cc ccccc}
        \toprule
        & \multicolumn{3}{c}{Optimal temps.} & \multicolumn{2}{c}{Members} & \multicolumn{2}{c}{Fixed temperatures} & \multicolumn{4}{c}{Oracles (labels used)} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-12}
        Stream & $T_L^*$ & $T_S^*$ & $T_L^*/T_S^*$ & Large & Small & Clean & Held-out & Corr.-wise & $B{=}128$ & $B{=}64$ & $B{=}16$ \\
        \midrule
        Clean (val) & 1.11 & 0.60 & 1.85 & 81.1 & 82.5 & 83.4 & 83.0 & 83.4 & 83.5 & 83.6 & 84.3 \\
        \midrule
        Speckle noise & 0.59 & 1.28 & 0.46 & 48.5 & 34.7 & 45.9 & 49.0 & 49.4 & 49.4 & 49.5 & 50.0 \\
        Gaussian blur & 0.62 & 2.02 & 0.31 & 29.5 & 20.4 & 26.7 & 28.9 & 29.6 & 29.7 & 29.7 & 30.1 \\
        Spatter & 0.96 & 0.58 & 1.68 & 52.1 & 54.1 & 58.3 & 57.2 & 58.3 & 58.4 & 58.6 & 59.2 \\
        Saturate& 0.93 & 0.69 & 1.35 & 65.0 & 65.3 & 68.8 & 68.6 & 68.9 & 69.0 & 69.2 & 69.9 \\
        \midrule
        Gaussian noise & 0.45 & 47.77 & 0.01 & 35.7 & 13.7 & 26.4 & 32.5 & 35.7 & 35.7 & 35.7 & 35.9 \\
        Shot noise & 0.49 & 4.71 & 0.10 & 34.2 & 15.6 & 27.4 & 32.5 & 34.1 & 34.2 & 34.2 & 34.5  \\
        Impulse noise & 0.43 & 37.19 & 0.01 & 36.9 & 13.5 & 26.9 & 33.5 & 36.9 & 36.8 & 36.9 & 37.0  \\
        Defocus blur & 0.63 & 1.87 & 0.34 & 31.6 & 22.4 & 28.9 & 31.1 & 31.7 & 31.6 & 31.8 & 32.2 \\
        Glass blur & 0.59 & 6.71 & 0.09 & 25.4 & 12.7 & 20.0 & 23.4 & 25.3 & 25.4 & 25.5 & 25.5 \\
        Motion blur & 0.63 & 1.87 & 0.34 & 36.0 & 25.7 & 33.4 & 35.7 & 36.2 & 36.3 & 36.4 & 36.9 \\
        Zoom blur & 0.79 & 1.02 & 0.78 & 33.4 & 28.9 & 33.7 & 34.7 & 34.7 & 34.8 & 34.8 & 35.4 \\
        Snow & 0.81 & 0.83 & 0.98 & 42.4 & 38.6 & 44.5 & 44.9 & 45.1 & 45.3 & 45.3 & 45.8 \\
        Frost & 0.57 & 0.90 & 0.64 & 55.0 & 45.8 & 54.4 & 56.7 & 56.7 & 56.9 & 56.9 & 57.3  \\
        Fog & 0.42 & 1.11 & 0.38 & 51.2 & 31.0 & 44.7 & 51.2 & 52.9 & 53.0 & 53.0 & 53.5 \\
        Brightness & 0.80 & 0.73 & 1.09 & 71.5 & 70.1 & 73.5 & 73.7 & 73.7 & 73.8 & 73.9 & 74.7  \\
        Contrast & 1.48 & 0.44 & 3.38 & 18.3 & 33.0 & 33.7 & 31.9 & 33.8 & 33.9 & 33.9 & 34.1 \\
        Elastic transform & 0.55 & 5.61 & 0.10 & 42.3 & 24.7 & 34.8 & 39.7 & 42.2 & 42.2 & 42.3 & 42.4 \\
        Pixelate & 0.56 & 1.67 & 0.34 & 40.2 & 20.7 & 35.2 & 39.5 & 40.3 & 40.5 & 40.6 & 40.8 \\
        JPEG compression & 0.83 & 0.86 & 0.96 & 52.2 & 49.8 & 54.0 & 54.5 & 54.5 & 54.6 & 54.7 & 55.2 \\
        \midrule
        Average (15 test) & 0.63 & 2.37 & 0.27 & 40.4 & 29.8 & 38.1 & 41.0 & 42.2 & 42.3 & 42.4 & 42.7 \\
        \bottomrule
    \end{tabular}}
\end{table*}


==> tables/1_temperatures/tab_temperatures_frozen_bn_vitb16_rn50v1.tex <==
\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{4.5pt}
    \caption{
    Temperatures and top-1 accuracy (\%) of the frozen Duo at severity 5 on episodic ImageNet-C. 
    Large / Small: \textbf{ViT-B/16 / ResNet-50}. 
    $T_L^*, T_S^*$: the temperatures minimizing the NLL of the Duo on each stream, which define the corr.-wise oracle, and $T_L^*/T_S^*$ their ratio. 
    Clean TS $T_L = 0.69$, $T_S = 1.46$; Held-out TS $T_L = 0.65$, $T_S = 1.01$. In the Average row, temperatures are geometric means.
    }
    \label{tab:temperatures:frozen_bn__vitb16_rn50v1}
    \label{tab:oracles:frozen_bn__vitb16_rn50v1}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l ccc cc cc ccccc}
        \toprule
        & \multicolumn{3}{c}{Optimal temps.} & \multicolumn{2}{c}{Members} & \multicolumn{2}{c}{Fixed temperatures} & \multicolumn{4}{c}{Oracles (labels used)} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-12}
        Stream & $T_L^*$ & $T_S^*$ & $T_L^*/T_S^*$ & Large & Small & Clean & Held-out & Corr.-wise & $B{=}128$ & $B{=}64$ & $B{=}16$ \\
        \midrule
        Clean (val) & 0.69 & 1.46 & 0.47 & 81.1 & 75.2 & 81.5 & 81.5 & 81.5 & 81.6 & 81.8 & 82.4 \\
        \midrule
        Speckle noise & 0.60 & 1.00 & 0.59 & 48.5 & 29.8 & 51.7 & 51.8 & 51.8 & 51.9 & 52.0 & 52.5 \\
        Gaussian blur & 0.63 & 1.11 & 0.57 & 29.5 & 11.2 & 31.2 & 31.3 & 31.3 & 31.3 & 31.4 & 31.8  \\
        Spatter & 0.71 & 0.89 & 0.79 & 52.1 & 39.7 & 55.9 & 56.5 & 56.7 & 56.8 & 56.8 & 57.4  \\
        Saturate & 0.77 & 0.96 & 0.81 & 65.0 & 58.6 & 68.2 & 68.6 & 68.7 & 68.8 & 68.9 & 69.6  \\
        \midrule
        Gaussian noise & 0.53 & 0.95 & 0.55 & 35.7 & 16.1 & 38.8 & 38.9 & 38.9 & 39.0 & 39.0 & 39.4 \\
        Shot noise & 0.56 & 0.93 & 0.60 & 34.2 & 16.9 & 37.6 & 37.9 & 37.9 & 37.9 & 38.0 & 38.4  \\
        Impulse noise & 0.51 & 0.94 & 0.55 & 36.9 & 16.7 & 40.3 & 40.2 & 40.3 & 40.4 & 40.4 & 41.0\\
        Defocus blur & 0.65 & 1.01 & 0.65 & 31.6 & 15.0 & 34.1 & 34.4 & 34.4 & 34.5 & 34.5 & 35.0 \\
        Glass blur & 0.75 & 0.91 & 0.83 & 25.4 & 15.3 & 28.0 & 28.4 & 28.6 & 28.7 & 28.8 & 29.1  \\
        Motion blur & 0.72 & 0.83 & 0.86 & 36.0 & 26.0 & 40.5 & 41.2 & 41.6 & 41.6 & 41.7 & 42.2 \\
        Zoom blur & 1.01 & 0.64 & 1.57 & 33.4 & 38.6 & 40.4 & 42.1 & 45.1 & 45.3 & 45.3 & 45.8 \\
        Snow & 0.72 & 0.85 & 0.85 & 42.4 & 34.2 & 47.2 & 48.0 & 48.4 & 48.5 & 48.5 & 49.1 \\
        Frost & 0.52 & 1.30 & 0.40 & 55.0 & 33.0 & 56.4 & 55.9 & 56.5 & 56.6 & 56.7 & 57.1  \\
        Fog & 0.54 & 0.80 & 0.68 & 51.2 & 47.9 & 62.6 & 62.9 & 62.8 & 62.9 & 63.0 & 63.5 \\
        Brightness & 0.74 & 1.07 & 0.69 & 71.5 & 65.3 & 73.6 & 73.9 & 73.9 & 74.0 & 74.0 & 74.7 \\
        Contrast & 0.49 & 0.75 & 0.65 & 18.3 & 16.8 & 30.0 & 29.8 & 29.8 & 29.8 & 29.8 & 30.1  \\
        Elastic transform & 1.01 & 0.70 & 1.45 & 42.3 & 44.1 & 48.0 & 49.2 & 51.4 & 51.5 & 51.5 & 52.1 \\
        Pixelate & 0.98 & 0.63 & 1.56 & 40.2 & 48.8 & 50.1 & 52.1 & 55.6 & 55.6 & 55.6 & 56.1 \\
        JPEG compression & 0.69 & 0.86 & 0.80 & 52.2 & 40.0 & 56.1 & 56.7 & 57.0 & 57.2 & 57.2 & 57.7  \\
        \midrule
        Average (15 test) & 0.67 & 0.86 & 0.78 & 40.4 & 31.6 & 45.6 & 46.1 & 46.8 & 46.9 & 46.9 & 47.4 \\
        \bottomrule
    \end{tabular}}
\end{table*}


==> tables/2_adapting_duos/tab_adaptation_modes__tent__vitb16_convnextt_bn__worst_shift_gate_nnn_bt256_beta0p25-0p5.tex <==
\begin{table*}[t]
    \centering
    \small
    \setlength{\tabcolsep}{3.5pt}
    \caption{Top-1 accuracy (\%) of each member alone and of the Duo, under each way of adapting. 
    Large / small: \textbf{ViT-B/16 / ConvNeXt-T}, adapted with Tent, on episodic ImageNet-C at severity 5. 
    Fixed TS combines the members with $T_L = 0.72$, $T_S = 0.94$, fitted on the four held-out corruptions pooled, on the frozen models' logits; the $\beta$ rows use our gate (\cref{eq:gate}). 
    Mean over 3 seeds. 
    }
    \label{tab:adaptation_modes:tent__vitb16_convnextt_bn__worst_shift_gate_nnn_bt256_beta0p25-0p5_recpair}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l c@{\hspace{4\tabcolsep}}ccc cccc cccc cccc@{\hspace{4\tabcolsep}}c}
        \toprule
        & & \multicolumn{3}{c}{Noise} & \multicolumn{4}{c}{Blur} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Digital} & \\
        \cmidrule(lr){3-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}
        Method & Clean & Gauss. & Shot & Impulse & Defocus & Glass & Motion & Zoom & Snow & Frost & Fog & Bright. & Contrast & Elastic & Pixel. & JPEG & Avg. \\
        \midrule
        \multicolumn{18}{l}{\textit{Frozen}} \\
        \quad Large & 81.1 & 35.7 & 34.2 & 36.9 & 31.6 & 25.4 & 36.0 & 33.4 & 42.4 & 55.0 & 51.2 & 71.5 & 18.3 & 42.3 & 40.2 & 52.2 & 40.4 \\
        \quad Small & 82.5 & 13.7 & 15.6 & 13.5 & 22.4 & 12.7 & 25.7 & 28.9 & 38.6 & 45.8 & 31.0 & 70.1 & 33.0 & 24.7 & 20.7 & 49.8 & 29.8 \\
        \quad Duo & 83.0 & 32.5 & 32.5 & 33.5 & 31.1 & 23.4 & 35.7 & 34.7 & 44.9 & 56.7 & 51.2 & 73.7 & 31.9 & 39.7 & 39.5 & 54.5 & 41.0 \\
        \midrule
        \multicolumn{18}{l}{\textit{Single model, own entropy (Tent)}} \\
        \quad Large adapts & 81.0 & 40.5 & 41.0 & 41.8 & 35.6 & 31.2 & 41.8 & 37.8 & 44.7 & 53.6 & 19.5 & 72.3 & 30.6 & 45.8 & 51.5 & 55.8 & 42.9 \\
        \quad Small adapts & 81.3 & 17.5 & 31.3 & 25.9 & 23.4 & 21.0 & 33.3 & 12.4 & 5.7 & 9.2 & 3.3 & 72.7 & 49.3 & 3.8 & 46.8 & 54.0 & 27.3 \\
        \midrule
        \multicolumn{18}{l}{\textit{Duo, own entropy}} \\
        \quad Large adapts & 83.0 & 39.6 & 40.2 & 41.2 & 34.6 & 28.9 & 40.8 & 38.1 & 46.7 & 55.0 & 36.9 & 74.1 & 36.6 & 42.9 & 50.7 & 56.9 & 44.2 \\
        \quad Small adapts & 82.8 & 34.6 & 40.0 & 39.3 & 32.0 & 26.9 & 41.5 & 27.9 & 28.9 & 27.4 & 13.0 & 75.1 & 47.9 & 27.9 & 48.8 & 56.8 & 37.9 \\
        \quad Both adapt, Fixed TS & 82.8 & 39.6 & 45.3 & 42.7 & 36.8 & 31.6 & 46.2 & 33.5 & 34.5 & 42.0 & 18.5 & 75.7 & 48.8 & 36.2 & 57.2 & 59.7 & 43.2 \\
        \quad Both adapt, DD $\beta{=}0.25$ & 82.7 & 41.8 & 45.2 & 44.0 & 37.0 & 32.5 & 46.1 & 38.5 & 42.3 & 53.5 & 19.5 & 75.6 & 49.4 & 44.8 & 57.1 & 59.5 & 45.8 \\
        \quad Both adapt, DD $\beta{=}0.5$ & 82.7 & 41.8 & 45.0 & 43.9 & 37.3 & 32.8 & 46.0 & 39.3 & 43.8 & 54.1 & 18.9 & 75.5 & 49.5 & 46.0 & 56.9 & 59.4 & 46.0 \\
        \midrule
        \multicolumn{18}{l}{\textit{Duo, Duo entropy}} \\
        \quad Large adapts & 83.0 & 25.9 & 40.6 & 39.9 & 39.2 & 9.3 & 39.6 & 39.9 & 24.0 & 58.1 & 7.3 & 75.1 & 52.0 & 21.9 & 59.0 & 59.8 & 39.4 \\
        \quad Small adapts & 82.8 & 22.0 & 27.1 & 36.7 & 34.7 & 17.5 & 21.6 & 8.7 & 11.6 & 61.4 & 68.2 & 76.0 & 2.4 & 46.6 & 53.2 & 59.2 & 36.5 \\
        \quad Both adapt, Fixed TS & 82.8 & 38.0 & 31.8 & 46.3 & 34.6 & 18.8 & 21.0 & 8.5 & 11.5 & 61.4 & 68.2 & 76.1 & 2.4 & 46.8 & 54.1 & 59.4 & 38.6 \\
        \quad Both adapt, DD $\beta{=}0.25$ & 82.9 & 39.4 & 39.3 & 45.9 & 34.6 & 27.4 & 37.0 & 28.0 & 39.1 & 61.5 & 69.1 & 76.2 & 2.7 & 46.7 & 55.3 & 59.5 & 44.1 \\
        \quad Both adapt, DD $\beta{=}0.5$ & 82.9 & 43.0 & 40.7 & 45.6 & 34.6 & 27.7 & 39.1 & 33.7 & 43.2 & 58.6 & 69.1 & 76.3 & 3.9 & 46.7 & 56.4 & 59.6 & 45.2 \\
        \bottomrule
    \end{tabular}%
    }
\end{table*}


==> tables/2_adapting_duos/tab_adaptation_modes__tent__vitb16_rn50v1_bn_gate_nnn_bt256_beta0p25-0p5.tex <==
\begin{table*}
    \centering
    \small
    \setlength{\tabcolsep}{3.5pt}
    \caption{Top-1 accuracy (\%) of each member alone and of the Duo, under each way of adapting. 
    Large / small: \textbf{ViT-B/16 / ResNet-50}, adapted with Tent, on episodic ImageNet-C at severity 5. 
    Fixed TS combines the members with $T_L = 0.65$, $T_S = 1.01$, fitted on the four held-out corruptions pooled, on the frozen models' logits; the $\beta$ rows use our gate (\cref{eq:gate}). 
    Mean over 3 seeds. 
    }
    \label{tab:adaptation_modes:tent__vitb16_rn50v1_bn_gate_nnn_bt256_beta0p25-0p5_recpair}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l c@{\hspace{4\tabcolsep}}ccc cccc cccc cccc@{\hspace{4\tabcolsep}}c}
        \toprule
        & & \multicolumn{3}{c}{Noise} & \multicolumn{4}{c}{Blur} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Digital} & \\
        \cmidrule(lr){3-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}
        Method & Clean & Gauss. & Shot & Impulse & Defocus & Glass & Motion & Zoom & Snow & Frost & Fog & Bright. & Contrast & Elastic & Pixel. & JPEG & Avg. \\
        \midrule
        \multicolumn{18}{l}{\textit{Frozen}} \\
        \quad Large & 81.1 & 35.7 & 34.2 & 36.9 & 31.6 & 25.4 & 36.0 & 33.4 & 42.4 & 55.0 & 51.2 & 71.5 & 18.3 & 42.3 & 40.2 & 52.2 & 40.4 \\
        \quad Small & 75.2 & 16.1 & 16.8 & 16.7 & 15.0 & 15.3 & 26.1 & 38.8 & 34.2 & 33.0 & 47.8 & 65.4 & 16.8 & 44.0 & 48.9 & 40.1 & 31.7 \\
        \quad Duo & 81.5 & 38.9 & 37.9 & 40.3 & 34.4 & 28.4 & 41.2 & 42.0 & 48.0 & 55.9 & 62.8 & 73.8 & 29.9 & 49.2 & 52.2 & 56.7 & 46.1 \\
        \midrule
        \multicolumn{18}{l}{\textit{Single model, own entropy (Tent)}} \\
        \quad Large adapts & 81.0 & 40.5 & 41.0 & 41.8 & 35.6 & 31.2 & 41.8 & 37.8 & 44.7 & 53.6 & 19.5 & 72.3 & 30.6 & 45.8 & 51.5 & 55.8 & 42.9 \\
        \quad Small adapts & 75.2 & 31.4 & 33.7 & 33.3 & 29.3 & 28.6 & 43.6 & 50.6 & 49.1 & 40.8 & 58.4 & 67.6 & 22.6 & 55.9 & 59.5 & 53.7 & 43.9 \\
        \midrule
        \multicolumn{18}{l}{\textit{Duo, own entropy}} \\
        \quad Large adapts & 81.5 & 42.3 & 43.1 & 43.8 & 37.7 & 33.4 & 45.3 & 44.4 & 49.5 & 54.7 & 55.8 & 74.3 & 36.1 & 51.3 & 58.1 & 59.2 & 48.6 \\
        \quad Small adapts & 81.5 & 43.2 & 43.7 & 44.8 & 39.1 & 34.8 & 48.1 & 50.1 & 54.0 & 57.0 & 65.7 & 74.5 & 30.0 & 56.2 & 57.6 & 59.5 & 50.6 \\
        \quad Both adapt, Fixed TS & 81.4 & 45.4 & 46.8 & 47.0 & 41.2 & 38.0 & 50.3 & 51.1 & 54.7 & 56.0 & 62.9 & 74.8 & 35.0 & 57.3 & 61.4 & 61.3 & 52.2 \\
        \quad Both adapt, DD $\beta{=}0.25$ & 81.4 & 45.4 & 46.8 & 47.0 & 41.2 & 38.0 & 50.5 & 51.8 & 54.9 & 56.0 & 64.9 & 74.8 & 35.1 & 57.8 & 61.7 & 61.3 & 52.5 \\
        \quad Both adapt, DD $\beta{=}0.5$ & 81.4 & 45.3 & 46.7 & 47.0 & 41.2 & 38.0 & 50.7 & 52.4 & 55.1 & 56.1 & 64.2 & 74.8 & 34.8 & 58.2 & 62.1 & 61.2 & 52.5 \\
        \midrule
        \multicolumn{18}{l}{\textit{Duo, Duo entropy}} \\
        \quad Large adapts & 81.5 & 46.5 & 48.7 & 48.3 & 47.3 & 47.0 & 54.9 & 54.8 & 44.2 & 59.7 & 67.6 & 75.5 & 56.4 & 61.0 & 66.4 & 64.6 & 56.2 \\
        \quad Small adapts & 81.5 & 44.1 & 44.2 & 45.6 & 39.2 & 33.5 & 47.2 & 46.8 & 52.2 & 58.6 & 65.9 & 74.5 & 36.0 & 53.4 & 56.7 & 59.2 & 50.5 \\
        \quad Both adapt, Fixed TS & 81.5 & 49.3 & 51.6 & 51.0 & 50.0 & 50.6 & 58.9 & 56.6 & 51.5 & 59.5 & 69.7 & 76.1 & 60.5 & 65.3 & 68.9 & 67.0 & 59.1 \\
        \quad Both adapt, DD $\beta{=}0.25$ & 81.5 & 44.6 & 50.3 & 49.9 & 49.4 & 47.9 & 58.3 & 55.3 & 48.4 & 60.9 & 69.6 & 76.1 & 59.9 & 64.9 & 68.8 & 66.8 & 58.1 \\
        \quad Both adapt, DD $\beta{=}0.5$ & 81.5 & 32.7 & 48.5 & 48.6 & 48.2 & 32.7 & 57.7 & 54.2 & 44.4 & 60.8 & 69.5 & 76.1 & 59.1 & 64.6 & 68.6 & 66.7 & 55.5 \\
        \bottomrule
    \end{tabular}%
    }
\end{table*}

